Advances and Open Challenges in Federated Foundation Models

The integration of Foundation Models (FMs) with Federated Learning (FL) presents a transformative paradigm in Artificial Intelligence (AI). This integration offers enhanced capabilities, while addressing concerns of privacy, data decentralization and computational efficiency. This paper provides a comprehensive survey of the emerging field of Federated Foundation Models (FedFM), elucidating their synergistic relationship and exploring novel methodologies, challenges, and future directions that the FL research field needs to focus on in order to thrive in the age of FMs. A systematic multi-tiered taxonomy is proposed, categorizing existing FedFM approaches for model training, aggregation, trustworthiness, and incentivization. Key challenges, including how to enable FL to deal with high complexity of computational demands, privacy considerations, contribution evaluation, and communication efficiency, are thoroughly discussed. Moreover, this paper explores the intricate challenges of communication, scalability and security inherent in training/fine-tuning FMs via FL. It highlights the potential of quantum computing to revolutionize the processes of training, inference, optimization and security. This survey also introduces the implementation requirement of FedFM and some practical FedFM applications. It highlights lessons learned with a clear understanding of our findings for FedFM. Finally, this survey not only provides insights into the current state and challenges of FedFM, but also offers a blueprint for future research directions, emphasizing the need for developing trustworthy solutions. It serves as a foundational guide for researchers and practitioners interested in contributing to this interdisciplinary and rapidly advancing field.

==> evaluation.tex <==
\label{sec:evaluation}
Participant contribution evaluation is crucial to the success of \methodname{} for the following reasons. 
Firstly, the intricate non-linearity and complexity of \methodname{} pose a challenge for stakeholders to understand the internal working mechanisms and decision making processes.
This lack of transparency can diminish trust and impede adoption, especially in safety-critical sectors like finance and healthcare \cite{li2023towards}. 
Secondly, the evaluation of \methodname{} contributes to an enhanced understanding of their strengths and weaknesses. For instance, the PromptBench benchmark \cite{zhu2023promptbench}  demonstrated that existing FMs are sensitive to adversarial prompts, thereby emphasizing the importance of prompt engineering for better model performance. 


%As a prospective technology to enhance system safety and build trust among FL stakeholders, evaluating \methodname{} has attracted substantial research interest from both the academic and the industry. 
Contribution evaluation in \methodname{} is more challenging compared to the current approaches for centralized FMs or traditional FL. Firstly, different from centralized FM evaluations, \methodname{} cannot directly assess the quality of the training data used due to privacy protection requirements.
Secondly, \methodname{} evaluation is limited by the resource constraints in terms of local computation and communication power of the FL clients involved. 
Thirdly, compared to traditional FL, \methodname{} evaluation can involve a large number of sequences, resulting in insufficient test coverage \cite{kuchnik2023validating}. 

There are a number of existing evaluation methods for traditional FL and centralized FMs, but few for \methodname{}. In this section, we discuss existing evaluation methods and envision promising research directions for designing new \methodname{} evaluation protocols. We present approaches which cover relevant works to evaluate the model performance, explain the prediction results, and provide insights into the contributions made by individual participants or data samples. 

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht!]
\centering
 \caption{Summary of Evaluations of Traditional FL Models} 
	\label{tab:evaluation}
\resizebox{1\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c} \toprule  
{\textbf {\begin{tabular}[c]{@{}l@{}}Evaluations of \\ Traditional FL Models \end{tabular}}} &  
{\textbf {\begin{tabular}[c]{@{}l@{}}Detailed Methods\\ \usym{1F5F8}: suitable  \end{tabular}}}  & \multicolumn{2}{c|}{\textsc{Stakeholders}} & \multicolumn{2}{c|}{\makecell[c]{\textsc{Threat} \\ \textsc{Models}} } & \multicolumn{3}{c|}{\makecell[c]{\textsc{Privacy} \\ \textsc{Protection} \\ \textsc{Targets}}} & \multicolumn{3}{c|}{\makecell[c]{\textsc{Privacy} \\ \textsc{Protection} \\ \textsc{Techniques}} } & \multicolumn{2}{c}{\makecell[c]{\textsc{Effectiveness} \\ \textsc{Metrics}} } \\ \cline {3-14}
& & S1 & S2 & A1 & A2 & P1 & P2 & P3 & T1 & T2 & T3 & E1 & E2   \\ \hline
\multirow{2}{*}{\makecell[c]{Client \& Sample \\ Contribution Evaluation}} & Influence-based     & \checkmark &&\checkmark &\checkmark  & \checkmark& & & \checkmark & & &\checkmark & \\ \cline{2-14} 
& Shapley value-based & \checkmark & \checkmark &\checkmark & &\checkmark & & &\checkmark  &\checkmark & &\checkmark &\checkmark \\ \hline 
\multirow{2}{*}{\makecell[c]{Feature Contribution\\ Evaluation}} & Model-Agnostic &  & \checkmark & & & & & && \checkmark  &\checkmark &\checkmark & \\ \cline{2-14} 
& Model-Specific&&\checkmark&\checkmark& && &\checkmark & &\checkmark & &\checkmark &   \\ \hline 
\end{tabular}
}

\raggedleft
\renewcommand\arraystretch{0.8}
\begin{tabular}{@{}lllll@{}}
\scriptsize S1: To FL Server & \scriptsize A1: Semi-Honest Participants &  \scriptsize P1: Raw Data     & \scriptsize T1: Differential Privacy   & \scriptsize E1: Post-Interpretation Performance   \\
 \scriptsize S2: To FL Client & \scriptsize A2: Malicious Participants            & \scriptsize P2: Data Distribution & \scriptsize T2: Homomorphic Encryption   & \scriptsize    E2: Faithfulness     \\
   &    &     \scriptsize P3: Label        & \scriptsize T3: Secure Multi-party Computation
\end{tabular}%

\end{table*}


\subsection{Contribution Evaluation for Traditional FL} 
\subsubsection{Client and Sample Contribution Evaluations} 
\
\par
\indent The performance of the global FL model largely depends on the quality of the local data. Client and sample contribution evaluation helps the FL server understand this by tracing back to local data, and is important to model aggregation. FL client and sample contribution evaluation methods can be divided into two main categories: 1) Shapley value (SV)-based evaluation, and 2) influence-based evaluation (Table \ref{tab:evaluation}).



\textbf{Shapley Value-based Evaluation}:  
SV-based evaluation methods provide insights into FL clients' data through evaluating their contributions to the performance of the final FL model. Existing SV-based evaluation methods mostly focus on improving computational efficiency, while maintaining SV estimation accuracy. The original SV method is prohibitively expensive since the required utility function evaluation grows exponentially with the number of FL participants. 

Existing FL evaluations based on efficient SV calculation can be divided into two categories: 1) accelerating within-round evaluations, and 2) reducing the number of rounds of sub-model evaluation. 
For the first approach, instead of re-training them from scratch, gradient-based SV \cite{nagalapatti2021game} and local embedding-based SV  \cite{fan2022fair} methods have been proposed to reconstruct sub-models. 
For the second approach, three main methods have been proposed. 
The first evaluates every possible sub-model as in the original SV setting based on gradient-based estimation \cite{song2019profit, wei2020efficient}. 
The second method leverages randomly sampled permutation evaluation \cite{wang2020principled,wang2022efficient} which produces the estimated SV of an FL participant as its expected contribution. 
However, since the number of selected permutations is fixed, potentially important permutations might be overlooked, resulting in inaccurate estimation. Thus, the third approach \cite{liu2022gtg,liu2022contribution} combines the guided Monte Carlo sampling technique and the within-round and between-round truncation techniques to prioritize sub-model permutations based on their importance. 

Another branch studies the problem of secure SV calculation under malicious settings. 
In \cite{zheng2022secure}, a two-server secure SV calculation protocol was proposed, which leverages a hybrid scheme to avoid ciphertext-ciphertext multiplications. Another work \cite{ma2021transparent} proposed a group-based SV computation scheme leveraging a blockchain-based secure framework with secure aggregation to protect participants' data privacy. 

\textbf{Influence-based Evaluation}: 
Though SV-based FL client and sample contribution evaluation considers the complex dependencies among clients, they are generally highly expensive to compute. 
Influence-based FL contribution evaluation methods have been proposed to efficiently evaluate the contribution of FL clients and their local data samples on FL model performance. 
Existing influence-based methods can be divided into two main branches. The first \cite{wang2019measure,zhang2022intrinsic} perturbs clients or their local samples to retrain FL models, and uses the difference in performance (\emph{e.g.}, test loss, test accuracy) between the new model and the original one to approximate client or sample contribution.  
However, since this method requires retraining of FL models on all clients' datasets or individual samples, the evaluation procedure is prohibitively expensive \cite{li2021efficient, koh2017understanding}. 

The second category uses influence function methods \cite{koh2017understanding} that leverage the second-order optimization technique to avoid the expensive retraining. 
An early approach leveraging influence functions in client contribution evaluation is Fed-influence \cite{xue2021toward}. 
To measure the influence of a client, Fed-influence sums up all sample influence values since there is an additive property of 
the influence function when measuring changes in test predictions \cite{koh2019accuracy}. However, this approach requires clients to  calculate the inverse of the Hessian matrix and transmit it, which incurs large computation and communication overhead. 
To reduce the overhead of influence approximation, emerging methods \cite{li2021efficient,li2021privacy, kwon2023datainf, li2021sample} leverage the Hessian vector product (HVP) to approximate the influence values. They are capable of achieving the linear operation costs, making them promising for practical adoption.  
 
   


\subsubsection{Feature Contribution Evaluation}
\
\par
\indent
\textbf{Model-Agnostic Evaluation}:
These methods treat an FL model as a black-box and attempts to measure the relevance of each feature to the learning task to filter out irrelevant ones. 
They leverage various statistical measures (\emph{e.g.}, mutual information, Gini-impurity, F-statistics \cite{cassara2022federated, li2021privacy1, pansecure}) to compute per-feature relevance scores.   
Another branch of methods use efficient gradient-based SV estimation approaches for feature contribution evaluation \cite{wang2019measure,wang2019interpret}. However, they methods require the FL server to know all the IDs of clients' features, which might violate clients privacy and make them unsuitable for practical vertical FL applications. 



% \subsection{Locally Interpretable Models}
% Feature-based interpretation methods aim to identify the contributions of each feature in the input towards a specific FL model prediction.

\textbf{Model Specific Evaluation}: 
% \textbf{Attention-based Evaluation.} 
The utilization of attention-based evaluation method enables the server to interpret which specific parts of inputs are leveraged by the global FL model. 
In \cite{chen2020federated}, a hierarchical attention mechanism is proposed which develops task-specific attentions to access personal feature correlations. 
Besides, a temporal attention layer is designed to evaluate cross-client temporal correlations at the FL server level. The final visualization of the attention weights can be used to determine which features the global model focuses for individual predictions. Another work, Flames2Graph \cite{younisflames2graph}, offers a personalized evaluation approach for the multivariate time series FL classification problem. It extracts and visualizes the essential sequences that highly activate network neurons, and constructs a temporal evolution graph to capture the temporal dependencies among them. 
Furthermore, \cite{li2023fedsdg,li2023efficient} proposed a federated feature selection approach, which introduces a Gaussian stochastic dual-gate based on the $l_0$ constraints to efficiently and privately approximate the probability of a feature being selected. 



% Prototypes \& Criticisms - using real data instances to explain the dataset distribution; ii) Counterfactual explanations - explaining a prediction by searching or generating some instances with different feature values that change the prediction to a predefined output. 

\subsection{Contribution Evaluation for Centralized FMs}
Existing evaluation approaches designed for FMs can be divided into: 1) model-based evaluation, and 2) training data-based evaluation. 

\subsubsection{Model-based FM Evaluation} 
\
\par
\indent
The initial objective of language models, particularly FMs, is to enhance language processing task performance (\emph{e.g.}, inference accuracy, robustness, trustworthiness). There are two common evaluation methods for FMs: 1) automated evaluation, and 2) human evaluation. 
% The language processing tasks include both understanding and generation. 

\textbf{Automated Evaluation}: 
Automated evaluation of FMs commonly adopts standard metrics or indicators and evaluation tools to assess model performance. These include accuracy, fairness, ROUGE \cite{lin2004rouge} and BERTScore \cite{zhang2019bertscore}. For instance, the BLEU score \cite{papineni2002bleu} has been leveraged to measure the similarity and quality between the text generated by the FM and the reference text in a machine translation task. 
Due to its simplicity and automatic computing, this evaluation metric is widely adopted by existing FM evaluation effort. In addition, with the development of FMs, more advanced automated evaluation techniques are emerging. For example, Lin et al. \cite{lin2023llm} proposed a unified multidimensional automated evaluation approach, LLM-EVAL, for domain conversations. PandaLM \cite{wang2023pandalm} trained an additional LLM to evaluate different models, which is suitable for reproducible and automated language model evaluation.  


\textbf{Human Evaluation}: 
Human evaluation aims to assess the quality and accuracy of FM-generated results through human participation. Different from automated evaluation, human evaluation focuses more on specific application scenarios and can provide more comprehensive results. Usually, evaluators consist of experts, researchers or the target users. Recent human evaluation methods involve tasks including generation, summarization and analogical reasoning tasks.  
Bubeck et al. \cite{bubeck2023sparks} conducted various human-crafted tests on GPT-4. They observed that GPT-4 performs close to or even exceeds human performance on various tasks. In practice, automated evaluation and human evaluation are considered for adoption on a case-by-case basis. 





\subsubsection{Training Data-based FM Evaluation} 
\
\par
\indent
During fine-tuning, the training data might not be equally important for a pre-trained FM. 
On the one hand, pre-trained FMs are prone to significant performance degradation in the presence of noisy data. This effect can be further amplified when noisy or harmful samples are highly influential to the model. 
On the other hand, specific knowledge embedded within some samples might have been extracted after some training rounds. Thus, they can be ignored afterwards without affecting final fine-tuned model performance. 
Therefore, it is important to identify noisy samples and important samples in the fine-tuning data to improve training efficiency and model performance. 
Jain et al. \cite{jain2023bring} evaluate FMs from the data-based perspective by eliminating the need for laborious labeling of new data. 
In \cite{schoch2023data}, an efficient SV-based data evaluation method has been proposed. It achieves this design goal through an efficient sampling-based method that aggregates SVs computed from subsets for valuation of the entire training set, and a value transfer method that leverages value information extracted from a simple classifier trained using representations from the target language model. DataInf \cite{kwon2023datainf} is a computationally efficient influence approximation method that is based on an easy-to-compute closed-form expression. It can be easily applied to FMs. 


\subsection{Contribution Evaluation for \methodname{}}
As for evaluating \methodname{}, so far, there have been few relevant works. 
The work \cite{xing2023fedlogic} proposed a logic rule learning approach to select the optimal chain-of-thoughts prompts for improving the interpretability of federated prompt selection for multi-domain FMs. They cast this problem as a bi-level program, and solve it through variational expectation maximization. 
The work \cite{zhao2023privacy} proposed to evaluate \methodname{} by comparing the performance of the federated parameter-efficient fine-tuned model with traditional centralized fine-tuning methods. 
FedIT \cite{zhang2023towards} leverages FL as the learning framework for FM instruction tuning and conducted studies on the widely used GPT-4 to exploit the heterogeneous and diverse sets of instructions.  
FedNLP \cite{lin2021fednlp} is a benchmark framework for evaluating FL methods on four common formulations of NLP tasks: text classification, sequence tagging, question answering and seq2seq generation. They proposed a universal interface between Transformer-based language models (e.g., BERT, BART) and FL methods under various non-IID partitioning strategies.

SV-based methods have been extensively employed in conventional FL scenarios to assess the contribution of each participant. However, applying SV-based methods to measure contributions in \methodname{} settings presents two notable challenges: 1) inference latency, and 2) compositional gap. 

\subsubsection{Inference Latency}
\
\par
\indent
Due to the substantial number of model parameters, directly utilizing SV-based methods for contribution evaluation in \methodname{} is impractical. The vast scale of participants, coupled with a large number of participation records, significantly amplifies the complexity and time-latency involved in both training and inference. The large model size further hinders the feasibility of incorporating timely contribution feedback to update and refine the utility of each participant, as is customary in traditional FL settings. This timely feedback plays a pivotal role in the participant selection process.

\subsubsection{Compositional Gap}
\
\par
\indent
FMs often grapple with the issue of a compositional gap, where they struggle to generate correct answers to compositional problems, even though they can correctly answer all their sub-problems \cite{press2022measuring}. Directly requiring contributions from FMs for each participant is currently beyond their capabilities. FMs cannot fully exploit the open-world knowledge encoded in them \cite{kang2023llms, dai2023uncovering}, making it challenging to assess the contribution of each participant or even each component under \methodname{} settings.


